Building Machine Learning Challenges for Anomaly Detection in Science

Scientific discoveries are often made by finding a pattern or object that was not predicted by the known rules of science. Oftentimes, these anomalous events or objects that do not conform to the norms are an indication that the rules of science governing the data are incomplete, and something new needs to be present to explain these unexpected outliers. The challenge of finding anomalies can be confounding since it requires codifying a complete knowledge of the known scientific behaviors and then projecting these known behaviors on the data to look for deviations. When utilizing machine learning, this presents a particular challenge since we require that the model not only understands scientific data perfectly but also recognizes when the data is inconsistent and out of the scope of its trained behavior. In this paper, we present three datasets aimed at developing machine learning-based anomaly detection for disparate scientific domains covering astrophysics, genomics, and polar science. We present the different datasets along with a scheme to make machine learning challenges around the three datasets findable, accessible, interoperable, and reusable (FAIR). Furthermore, we present an approach that generalizes to future machine learning challenges, enabling the possibility of large, more compute-intensive challenges that can ultimately lead to scientific discovery.

==> notes.tex <==
Deadlines
Submit to Nature Communications
Deadline for completed draft: November 25th
Documents the challenge by November 14th
Aim Qualifications section by November 25th
Internal of the document until December 6th
Share with institutes and get comments by January 10th
Final Comments by January 24th 

Author list
3 tiers: Organizers, report editors, endorsers

%10 Pages (excluding references)
%December 1st proposal for going forward
%Presenting this problem 

Outline
Introduction (follow the workshop proposal)
Discusses the Motivation
Lists a bunch of metrics for success
3 Challenges
 - Challenges Section, or each as a section (<Institute> Challenge: <name of challenge>)?
Qualifications: FAIR, aligned across the challenges
Conclusions 


% Present some slides on the Neurscience forecasting challenge by January 10th


